On the Chabauty space of $\textrm{PSL}_2(\mathbb{R})$, I: lattices and grafting

This is the first of two papers on the global topology of the space $\textrm{Sub}(G)$ of all closed subgroups of $G=\textrm{PSL}_2(\mathbb{R})$, equipped with the Chabauty topology. In this paper, we study the spaces of lattices and elementary subgroups of $G$, and prove a continuity result for conformal grafting of (possibly infinite type) vectored orbifolds that will be useful in both papers. More specifically, we first identify the homotopy type of the space of elementary subgroups of $G$, following Baik-Clavier. Then for a fixed finite type hyperbolizable $2$-orbifold $S$, we show that the space $\textrm{Sub}_S(G)$ of all lattices $\Gamma < G$ with $\Gamma \backslash \mathbb{H}^2 \cong S$ is a fiber orbibundle over the moduli space $\mathcal M(S)$. We describe the closure $\overline{\textrm{Sub}_S(G)}$ in $\textrm{Sub}(G)$ and show that $\partial \textrm{Sub}_S(G)$ has a neighborhood deformation retract within $\overline{\textrm{Sub}_S(G)}$. When $S$ is not one of finitely many low complexity orbifolds, we show that $\overline{\textrm{Sub}_S(G)}$ is simply connected. In the simplest exceptional case, when $S$ is a sphere with three total cusps and cone points, we show that $\overline{\textrm{Sub}_S(G)}$ is a (usually nontrivial) lens space. Finally, we show that when $(X_i,v_i) \to (X_\infty,v_\infty)$ is a (possibly infinite type) smoothly converging sequence of vectored hyperbolic $2$-orbifolds, and we graft in Euclidean annuli along suitable collections of simple closed curves in the $X_i$, then after uniformization, the resulting vectored hyperbolic $2$-orbifolds converge smoothly to the expected limit. As part of the proof, we give a new lower bound on the hyperbolic distance between points in a grafted orbifold in terms of their original distance.

==> backup_of_proof.tex <==
\subsection{Global distance estimates (old version)}

In this section, we establish the following proposition, which relates the hyperbolic metric on a grafted orbifold with the  original hyperbolic metric, at least outside of the standard collars of the grafting curves. 

\begin{proposition}\label{prop: globalesstimates}
Given $\LLL$, there is a homeomorphism
$$\eta : [0,\infty] \longrightarrow [0,\infty], $$
 with $\eta(\infty)=\infty$ as follows. Suppose that $X$  is a hyperbolic $2$-orbifold, $\SSS$  is a collection of admissible geodesics on $X$ which satisfy $$\ell(c) \le \LLL  \quad \forall c\in \SSS.$$ Then, for all $L: \SSS \longrightarrow [0,\infty]$ and  for all $x,y\in X$ that lie outside the  standard collars of all curves in $\SSS$, we have
$$d_{(X_L)^{hyp}}\big (\iota(x),\iota(y)\big ) \geq \eta\big (d_X(x,y)\big ).$$
\end{proposition}

The idea of the proof is as follows. First assuming that $X$ is a surface, i.e. has no cone points, we will construct an explicit intermediate hyperbolic surface $Y$ by shrinking the length parameters of the grafting curves in Fenchel-Nielsen coordinates.
In Claim \ref{claim: quasiconformal map from XL to Y}, we will use \cite{buser2014quasiconformal} to find a $K$-quasiconformal map from $X_L$ to $Y$.  
Quasiconformal maps distort distances in a controlled way (see \cite[ Theorem 4.4.1]{hubbard}) so the proof will be complete if we can compare distances in $X$ to those in $Y$. 
This is done in Claim \ref{claim: Lipschitz map from X to Y}. 
Finally, if $X$ is an orbifold we use its surface cover to reduce Proposition \ref{prop: globalesstimates} to the case that $X$ is a surface. \todo{A: don't we just want a finite cover that resolves the cone points in the convex core of the grafting curves?}
 
\medskip
 
Let $X$ be a surface. Let $\LLL,\SSS,L$ be as in the proposition. By Theorem \ref{thm: pantsdecomps}, $X$ has a geodesic pair of pants decomposition. That is, there is a collection of geodesics $\PPP$ such that $X\dblsetminus \PPP$ consists of pair of pants, flares and halfspaces with geodesic boundaries. A closer look at the proof of Theorem \ref{thm: pantsdecomps} shows that $\PPP$ may be chosen to include $\SSS$.

Extend $L$ to a function $L:\PPP \to [0,\infty]$ by setting $L(c)=0$ for curves in $\PPP \setminus \SSS$. 
Using Fenchel-Nielsen coordinates, we build a new surface $Y$, by setting its twisting parameters to be as in $X$, and its length parameters to be $\ell_Y(c) = \frac{\ell_X(c)}{1 + \frac{2}{\pi}L(c)}$ for every $c\in \PPP$.

\begin{claim} \label{claim: quasiconformal map from XL to Y} 
The exists $K=K(\LLL)$ and a $K$-quasiconformal map $f:X_L\to Y$. Moreover, on each component $P\subseteq X\dblsetminus \PPP$ the map $f\circ \iota$ is locally $K$-bi-Lipschitz on the complement in $P$ of the reduced collars of the boundary curves of $P$ that belong to $\SSS$.
\end{claim}

\begin{proof}
We will build the map $f$ and verify its properties separately on each component $P$ of $X\dblsetminus \PPP$.

\textbf{Case 1. $P$ is a pair of pants.} It will be useful to introduce here some notation (similar to \cite{buser2014quasiconformal}). For $l_1,l_2,l_3\ge 0$, let $\bfP_{l_1,l_2,l_3}$ be the hyperbolic pair of pants with boundary curves (or cusps) $c_1,c_2,c_3$ of lengths $l_1,l_2,l_3$ respectively. 
Let $b_i$ be an equidistant curve (or horocycle) of $c_i$ in $\bfP_{l_1,l_2,l_3}$ of length $\lambda_i$. Then, we denote by $\bfP_{l_1,l_2,l_3}^{\lambda_1,\lambda_2,\lambda_3}$ the pair of pants in $\bfP_{l_1,l_2,l_3}$ bounded by $b_1,b_2,b_3$.

Assume $P \subseteq X\dblsetminus \PPP$ is a pair of pants with boundary curves $c_1,c_2,c_3$. If we set $\ell_i=\ell_X(c_i)$, we get $P\simeq \bfP_{\ell_1,\ell_2,\ell_3}$. Let $P_L$ be the Euclidean/hyperbolic pair of pants obtained by attaching the Euclidean cylinders $C_{c_i+}$ of width $L(c_i)$ to each boundary curve of $P$. 
Let $Q$ be the corresponding pair of pants in $Y$. Setting $$\ell_i'=\ell_Y(c_i)=\frac{\ell_i}{1 + \frac{2}{\pi}L(c_i)}$$ we get $Q\simeq \bfP_{\ell'_1,\ell'_2,\ell'_3}$. 
We wish to build a quasiconformal map $P_L\to Q$ which is boundary coherent, i.e, sends the boundary curves of $P_L$ to those of $Q$ so that they agree on their natural parametrizations. We do so by passing through a third pair of pants $P_L\to R\to Q$ using \cite[Theorem 5.1]{buser2014quasiconformal}.

We set parameters $\ell''_i,\ell^*_i$ for $i=1,2,3$ as follows: if $c\in \SSS$ set $\ell''_i=0$ and $\ell^*_i=\tfrac{2}{\pi}\ell_i$ while if $c\notin \SSS$ set $\ell''_i=\ell_i^*= \ell_i=\ell'_i$.
Consider the pair of pants $R=\bfP_{\ell''_1,\ell''_2,\ell''_3}$ and its subsurface $R^*=\bfP_{\ell''_1,\ell''_2,\ell''_3}^{\ell^*_1,\ell^*_2,\ell^*_3}$. 
By applying \cite[Theorem 5.1]{buser2014quasiconformal} successively for each curve $c_i\in\SSS$, we get a $K$-quasiconformal boundary coherent map $f_1:P\to  R^*$ with $K=K(\LLL)$.

If $c_i\in\SSS$ the connected component $E_i$ of $R \setminus R^*$ containing the curve $c_i$ is isometric to $\bbS^1_1\times [\frac{\pi}{2\ell_i},\infty)$ with the metric $ds^2=\frac{1}{y^2}(dx^2+dy^2)$. We extend $f_1$ conformally to the grafted cylinders $C_{c_i}$ as follows. 
The grafted cylinder $C_{c_i}$ is identified with $\bbS^1_{\ell_i}\times [0, L(c_i)]$, by scaling and translating the second coordinate we can conformally identify it with the subannulus $$\bbS^1_{1}\times \left[\frac{\pi}{2\ell_i},\frac{\tfrac{\pi}{2}+L(c_i)}{\ell_i}\right]\subseteq E_i.$$
Note that the boundary curve $\bbS^1_1\times \{\tfrac{\pi}{2}+L(c_i)/\ell_i\}$ is a horocycle of length 
\begin{equation}\label{eq: boundary curve length}
    \lambda_i=\frac{\ell_i}{\tfrac{\pi}{2}+L(c_i)}=\frac{2}{\pi}\ell'_i.
\end{equation}
This enables us to extend $f_1:P\to R^*\subseteq R$ to a map $f_1:P_L \to R^{**}:=\bfP_{\ell''_1,\ell''_2,\ell''_3}^{\lambda_1,\lambda_2,\lambda_3}\subset R$, where $\lambda_i$ are those defined above for $c_i\in \SSS$ and $\lambda_i=\ell''_i$ if $c_i\notin \SSS$. 

In view of the equality \eqref{eq: boundary curve length}, We can apply \cite[Theorem 5.1]{buser2014quasiconformal} to get a boundary coherent $K$-quasiconformal map $f_2:Q\to R^{**}\subseteq R$. 
Finally, the composition $f_P=f_2^{-1}\circ f_1$ is the desired conformal map $f_P:P_L\to Q$.

Next we show that $f_P:P_L\to Q$ is $K$-bi-Lipschitz outside the standard collar neighborhoods of the curves $c_i\in\SSS$. 
In $\bfP_{l_1,l_2,l_3}$ let the \emph{reduced collar} $\RC(c_i)$ be the annulus bounded by $c_i$ and the equidistant curve (or horocycle) of length $1+\frac{1}{4}l_i^2$, if $l_i\le 2$, and $\RC(c_i) = \emptyset$ if $l_i \geq 2$.  
For $0<l_i\le 2$, $\RC(c_i)$ can also be defined as the neighborhood of $c_i$ in $\bfP_{l_1,l_2,l_3}$ with radius $\ln (\frac{2}{l_i})$.  
Note that $\RC(c_i)$ is contained in the standard collar $A_{c_i}$ around $c_i$, defined in \S\ref{sec: collarsec}, since $$\ln (\frac{2}{l_i}) < \sinh ^{-1} (\frac{1}{\sinh(2 l_i)})$$ if $l_i\le 2$.
By \cite[Theorem 5.1]{buser2014quasiconformal} the map $f_1: P \to R$ maps reduced collars to reduced collars and is $K$-bi-Lipschitz on $P \setminus \bigcup_{i:c_i\in \SSS} \RC(c_i)$. 
Similarly, the map $f_2: Q \to R$ is $K$-bi-Lipschitz on $Q\setminus \bigcup_{i:c_i\in \SSS} \RC(c_i)$. 
The two restricted maps have the same image, namely $R\setminus \bigcup_{i:c_i\in \SSS} \RC(c_i)$.
Thus $P \setminus \bigcup_{i:c_i\in \SSS} \RC(c_i) \to Q$ is $K^2$-bi-Lipschitz.
In particular, the map from $P \setminus \bigcup_{i:c_i\in \SSS} A_{c_+} \to Q$ is uniformly bi-Lipschitz, since the standard collar $A_{c_i} \supset \RC(c_+)$. 

\textbf{Case 2. $P$ is a flare.}
Let $P \subseteq X \dblsetminus \PPP$ be a flare component, and let $c=\partial P$ be its boundary curve. Let $P_L$ be the grafted Euclidean/hyperbolic flare, i.e. the union of $P$ and the Euclidean cylinder $C_c$ of length $L(c)$. Let $Q\subseteq Y\dblsetminus \PPP$ be the corresponding flare in $Y$. Denote $$\ell = \ell_P(c) \text{ and }\ell':=\ell_Q(c)=\frac{\ell}{1+\tfrac{2}{\pi}L(c)}.$$ 
Parametrizing $P = \bbS^1 _ \ell \times [0, \frac{\pi}{2})$ and $C_c = \bbS^1 _ \ell \times [-L(c), 0]$ we see that $P_L$ can be conformally parametrized by $\bbS^1_\ell\times [-L(c),\frac{\pi}{2})$. Translating the second coordinate by $L(c)$ and scaling both by $\frac{1}{1+2L(c)/\pi}$, we get a conformal map $f_P:P_L\to \bbS^1_{\ell'}\times [0,\frac{\pi}{2})$. The range of the map is the conformal parametrization of $Q$.\todo{A: odd to say range=param} Thus we get a conformal map $f_P:P_L \to Q$.

Let us show that the map $f_P$ is $4$-bi-Lipschitz on $P$. %\tinytodo{might as well include the bilipschitz constant, since it's important that it's uniform, and the constant is like 4 or something}

In coordinates, the image of a point $(x,y)\in \bbS^1_\ell\times [0,\pi/2) \simeq P \subseteq P_L$ under the map $f_P$ is the point $$f_P(x,y)=\big(x, \tfrac{L(c)+y}{1 + \frac{2}{\pi}L(c)}\big).$$
To compute the metric distortion we work in coordinates. The hyperbolic metric at the point $(x,y)$ scaled by $1/\sec(y)$ gives the Euclidean metric; the map $f_P$ then scales the Euclidean metric by $\frac{1}{1 + \frac{2}{\pi} L}$; and finally by scaling it again by the secant of the second coordinate of $f_P(x,y)$ we get the hyperbolic metric at $f_P(x,y)$.
Putting them together we get that the metric distortion at $(x,y)$ is given by
\[ \frac{1}{\sec(y)}\cdot \frac{1}{1 + \frac{2}{\pi} L} \cdot \sec(\tfrac{L(c)+y}{1 + \frac{2}{\pi}L(c)})  .\]
By using 
$$\frac{1}{2} \cdot \frac{1}{\frac{\pi}{2} -y} \leq \sec(y) \leq 2 \cdot  \frac{1}{\frac{\pi}{2} -y},$$ we get that the distance distortion of $f_P$ is within $4=2\cdot 2$ of
\[ \left(\frac{1}{
\frac{1}{\frac{\pi}{2}-y}
}\right)\cdot
\left(\frac{1}{1 + \frac{2}{\pi} L}\right)
    \cdot\left(
     \frac{1}{\frac{\pi}{2}-\frac{L(c)+y}{1 + \frac{2}{\pi}L(c)}} \right) 
=\frac{ \frac{\pi}{2}-y }{\frac{\pi}{2}(1 + \frac{2}{\pi} L(c)) -L(c) -y} = 1.\]
Hence, it is $4$-bi-Lipschitz.
\medskip

\textbf{The map $f:X_L \to Y$.} 
The maps $f_P:P_L\to Y$ constructed on each component of $P \subset X\dblsetminus \PPP$ are boundary coherent, and so they can be glued together to get a map $f:X_L \to Y$. Since each of the maps $f_P$ is $K$-quasiconformal, so is $f$. Moreover, each $f_P$ is $K$-bi-Lipschitz on the complement in $P$ of the reduced collars of curves in $\SSS$ as required.
\end{proof}

\begin{claim} \label{claim: Lipschitz map from X to Y} 
Let $f:X_L\to Y$ be the map constructed in Claim \ref{claim: quasiconformal map from XL to Y}, there exists $K'$ such that for all $x_1,x_2\in X$ which are outside the standard collar neighbrohood of curves in $\SSS$, we have 
\[  d_Y(f\circ \iota (x_1), f\circ \iota(x_2)) \ge  \frac{1}{K'} d_X(x_1,x_2).\]
\end{claim}

\begin{proof}
Let $y_i = f\circ \iota (x_i) \in Y$. Let $\gamma$ be the geodesic in $Y$ connecting $y_1$ and $y_2$. The geodesic $\gamma$ can be broken into subarcs $\alpha_1,\ldots,\alpha_n$ each is either in $Q\setminus \bigcup_{\partial Q \supset c\in\SSS} \RC(c)$ for some component $Q\subset Y\dblsetminus \PPP$ or in $\RC(c)$ for some $c\in \SSS$.
Note that the endpoints $\partial \alpha_i$ of each subarc are outside the reduced collars of curves in $\SSS$ in $Y$. Since $f$ maps the reduced collars of $X$ to those of $Y$, we see that $(f\circ \iota)^{-1}(\partial \alpha_i)$ are points of $X$ outside the reduced collar neighborhood of curves in $\SSS$.
For each $\alpha_i \subset Y$ we will find a curve $\beta_i \subset X$ such that $f\circ \iota (\partial \beta_i) = \partial \alpha_i$, satisfying $\length(\alpha_i) \ge \frac{1}{K'}\length(\beta_i)$ for all $i=1,\ldots,n$.


We divide into cases:

\textbf{Case 1.} If $\alpha_i$ is outside the reduced collars, let $\beta_i=(f\circ \iota)^{-1}\circ \alpha_i$. Then, by Claim \ref{claim: quasiconformal map from XL to Y}, $f\circ \iota$ is locally a $K$-bi-Lipschitz map on $\alpha_i$, and we get $\length(\alpha_i) \ge \frac{1}{K}\length(\beta_i)$.

\textbf{Case 2.} If $\alpha_i \subseteq \RC(c)$ for some $c\in\SSS$. Then, there are two cases to consider:

\textbf{Case 2.1.} If $\alpha_i$ is an essential arc, that is, $\partial \alpha_i$ is on two different components of $\RC(c)$. Recall that the distance across the reduced collar is $2\ln(2/\ell(c))$. Then, 
\[\length(\alpha_i) > 2\ln (2/\ell_Y(c)) > 2\ln(2/\ell_X(c)).\] 
Setting $K_0=\frac{1}{4\ln 4} + 1$ it is easy to verify that since $\ell_X(c)<\tfrac{1}{2}$ we have
\[ 2\ln(2/\ell_X(c))
> \frac{1}{K_0}(2\ln(2/\ell_X(c)) + \ell_X(c))
\]
Finally, let $\{q_1,q_2\} = (f\circ \iota)^{-1}(\partial \alpha_i)$. Let $\beta_i$ be the arc in $\RC_X(c)$ which is the union of the two geodesics from $q_1,q_2$ to their nearest point projections on $c$, and the subarc on $c$ connecting their projections. Hence $\length(\beta_i)$ is shorter than twice the radius of the reduced collar + the length of the curve $c$.
Putting everything together gives
\[\length(\alpha_i) > \frac{1}{K_0}(2\ln(2/\ell_X(c)) + \ell_X(c)) > \frac{1}{K_0}\length(\beta_i).\]

\textbf{Case 2.2.} If $\alpha_i$ is an inessential arc.  Let $\alpha_i'$ be the shortest path in $\partial \RC(c)$ connecting $\partial \alpha_i$. Then, using $\ell(c)<\frac{1}{2}$ one can verify, for example by considering the length distortion obtained by projecting each point of $\alpha_i$ to the closest point in $\partial \RC(c)$, that there \todo{A: $K_1$ is universal for all $i$? Or for each $i$ there is a $K_1$?} exists\footnote{E.g one can take $K_1 = 1/\cos(\Sec^{-1}(\ln (4))))$} $K_1$ such that $$\length(\alpha_i)> \frac{1}{K_1}\length(\alpha_i'). $$
Letting $\beta_i =(f\circ \iota)^{-1}\circ \alpha_i'$ by Case 1 we have:
$$\length(\alpha_i)> \frac{1}{K_1}\length(\alpha_i')>\frac{1}{KK_1}\length(\beta_i). $$

Set $K'=\max\{K,K_0, KK_1\}$, the proof is complete since
\[ d_Y(y_1,y_2) = \sum_{i=1}^n \length(\alpha_i) \ge \sum_{i=1}^{n} \frac{1}{K'}\length(\beta_i) \ge \frac{1}{K'}d(x_1,x_2).\]
\end{proof}

\begin{lemma}\label{lem: smooth cover with double covers}
Let $X$ be an orbifold, and let $\SSS$ be a collection of disjoint geodesic curves. Then, there exists a (possibly infinite) surface cover $\hat X$ of $X$ such that each lift of $c\in \SSS$ double covers $c$.
\end{lemma}

\begin{proof}
Extend $\SSS$ to a generalized pair of pants decomposition $\PPP$.
If we show that each pair of pants (or flare) $P$ has a surface cover $\hat P$ in which each lift of $c\subseteq \partial P$ double covers $c$, then we get the desired cover $\hat X$ as the ``tree of spaces'' formed by gluing together the covers $\hat P$ of each $P$ along their matching boundaries.
Thus it suffices to show that such a cover $\hat P$ of $P$ exists.

If $P$ is a flare, then $\hat P$ is simply the double cover of $P$.
If $P$ is a generalized pair of pants, then its fundamental group is given by 
\[ \pi_1(P) = \left<x_1,x_2,x_3 \mid x_1x_2x_3,\; {x_1}^{n_1},\; {x_2}^{n_1},\; {x_3}^{n_3}\right>\]
where $n_1,n_2,n_3\in \NN \cup \{\infty\}$ and at least one of them is $\infty$.
The boundary curves of $P$ correspond to (conjugacy classes of) the generators $x_i$ with $n_i=\infty$.
Thus, $\pi_1(P)$ has the quotient
\[ H= \left<x_1,x_2,x_3 \mid x_1x_2x_3,\; {x_1}^{n_1'},\; {x_2}^{n_1'},\; {x_3}^{n_3'}\right>\]
where $n_i' = n_i$ if $n_i<\infty$ and $n_i'=2$ otherwise.
Since $H$ is a triangle group, we know that $x_1,x_2,x_3$ are elements of order $n_i'$ in $H$. 
This means that in the regular cover $\hat P$ of $P$ that corresponds to $\pi_1(P)\to H$ each lift of a cone point is smooth, and each lift of a boundary component is a double cover.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop: globalesstimates}]
Let $X$ be a hyperbolic orbifold. Let $\SSS$ be a collection of curves in $X$ with $\ell(c)<\tfrac{1}{4}$ for all $c\in \SSS$. By Lemma \ref{lem: smooth cover with double covers} there exists a surface cover $q:\hat X\to X$. Let $\hat\SSS$ be the lifts to $\hat X$ of all curves in $\SSS$. 

Note the following: 
\begin{enumerate}
    \item If $\hat c\in \hat \SSS$ then $\ell_{\hat X}(\hat c)<\tfrac{1}{2}$. 
    \item If $\hat{c}$ is a lift of $c$ then $q(A_{\hat c})\subset A_c$.
    \item If we set $\hat L : \hat \SSS \to [0,\infty]$ by $\hat L ( \hat c) = L (q(\hat c))$ for every $\hat c\in \hat \SSS$, then $\hat X_{\hat L}$ is a cover of $X_L$.
    \item For all $x,y\in X$, we have $d_X(x,y) = \min d_{\hat{X}}(\hat{x},\hat{y})$ where the minimum is taken over all lifts $\hat{x}, \hat{y} \in \hat X$ of $x,y$ respectively. Similarly, $d_{(X_L)^{\hyp}} (x,y) =\min d_{(\hat X_{\hat L})^{\hyp} } (\hat x,\hat y)$.
\end{enumerate} 
It follows that it suffices to prove the proposition for the surface $\hat X$, under the modified assumption that the curves in $\hat \SSS$ have length $<\tfrac{1}{2}$. 

By the reduction above, let us assume that $X$ is a surface and that curves in $\SSS$ have length $<\tfrac{1}{2}$.
Construct the surface $Y$ as above, and the map $f:X_L\to Y$ as in Claim \ref{claim: quasiconformal map from XL to Y}.

Let $x_1,x_2 \in X$ be outside the standard collar neighborhoods of curves in $\SSS$.
By Claim \ref{claim: Lipschitz map from X to Y} there exists $K'$ such that 
\begin{equation} \label{eq: f iota distorsion}
    d_Y(f\circ\iota(x_1),f\circ \iota(x_2)) \ge \frac{1}{K'} d_X(x_1,x_2).
\end{equation} 
In Claim \ref{claim: quasiconformal map from XL to Y}, we saw that $f$ is $K$-quasiconformal, hence it has a $K$-quasiconformal inverse. By \cite[Theorem 4.4.1]{hubbard} there exists a homeomorphism $\delta_K:\RR_+ \to \RR_+$ such that 
\[ d_{(X_L)^{\hyp}}(f^{-1}(y_1),f^{-1}(y_2))\ge \delta_K ( d_Y(y_1,y_2))\]
for all $y_1,y_2 \in Y$.
In particular, for $y_i = f\circ \iota (x_i)$ we get 
\[ d_{(X_L)^{\hyp}}(\iota(x_1),\iota(x_2)) \ge \delta_K(d_Y(f(x_1),f(x_2)))\ge   \delta_K(\frac{1}{K'}  d_X(x_1,x_2)).\]
The proof is complete if we take $\eta (s)= \delta_K( s/K')$.
\end{proof}


% ################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################################

In this section, we establish the following proposition, which relates the hyperbolic metric on a grafted orbifold with the  original hyperbolic metric, at least outside of the standard collars of the grafting curves. 

\begin{proposition}\label{prop: globalesstimates}
Given $\mathcal L$, there is a function
$$\eta : [0,\infty] \longrightarrow [0,\infty], $$
 with $\eta(t)\to \infty$ as $t\to \infty$, as follows. Suppose that $X$  is a hyperbolic $2$-orbifold, $\mathcal S$  is a finite collection of simple closed geodesics on $X$, $L: \mathcal S \longrightarrow [0,\infty]$ is a function, and $X_L$ is  the corresponding grafted orbifold, as defined in the beginning of \S \ref{sec: graftingsec}.   Suppose that we have 
$$\ell(c) \leq \mathcal L \ \ \forall c\in \mathcal S.$$
Then for all $x,y\in X$ that lie outside the  standard collars of all curves in $\mathcal S$, we have
$$d_{(X_L)^{hyp}}\big (\iota(x),\iota(y)\big ) \geq \eta\big (d_X(x,y)\big ).$$
\end{proposition}

The idea of the proof is to construct an explicit hyperbolic $2$-orbifold that is $K$-quasiconformal to $X_L$, for some fixed $K=K(\mathcal L)$, by shrinking the length parameters of the grafting curves in Fenchel-Nielsen coordinates.
The proposition will then follow from a standard estimate for the length distorsion of $K$-quasiconformal maps, see Theorem 4.4.1 in \cite{hubbard} which for convenience, we state here:
 
 \begin{theorem}[\cite{hubbard} Theorem 4.4.1] \label{thm: Hubbard}  There exists a function $\delta_K : \RR_+ \to \RR_+$  such that if $X$ and $Y$ are hyperbolic Riemann surfaces with hyperbolic metrics $d_X, d_Y$ and $f: X \to Y$ is $K$-quasiconformal then 
\[d _Y(f(x_1), f(x_2)) < \delta_K (d_X(x_1, x_2)) .\]
\end{theorem} 

Notice that in the proof we will make use of the fact that these orbifolds have all the grafting curves contained in some compact subsurface. That is, there may be singularities far out in the orbifold somewhere, but we have control on the parts of the surface where we graft. 


\begin{proof}
[Proof of Proposition \ref{prop: globalesstimates}]
We will first write the proof where $X$ is a surface, and then discuss how to modify the proof to the case where $X$ is an orbifold and contains cone points. 

Since a pants decomposition is a maximal collection of curves on a surface, we may extend $\SSS$ to a pants decomposition of some compact subsurface of $X$, see Theorem \ref{thm: pantsdecomps}.  We may do this in such a way that each side of every $c \in \SSS$ is adjacent in $X$ to either a pair of pants or to a flare.  For each curve $c \in \SSS$ we will describe a way to build a quasiconformal map from an adjacent pair of pants (or flare) union a Euclidean annulus, to a hyperbolic pair of pants (or flare) based on results of \cite{buser2014quasiconformal}.   Doing this for every $c \in \SSS$ will give a quasiconformal map from the grafted surface (which is piecewise hyperbolic/ Euclidean) to a hyperbolic surface. 

\textbf{ Case 1: $c$ is adjacent to pants} 

Choose some $c \in \SSS$ and a side $c_+$ adjacent to a pair of pants $P$.  Along $c$ graft an annulus, $A$, with length $L(c)$, so that the circumference of $A$ is $\ell(c)$.  Thus we have a pair of pants $P \cup A$ where the lengths of the boundary curves are $\ell_1, \ell_2$ and $\ell(c)$.  We denote $\varepsilon := \ell(c)$. 

Now consider a pair of pants, $Q$ with boundary lengths $\ell_1, \ell_2$ and $\varepsilon ' = \frac{\varepsilon}{1 + \frac{2}{\pi}L}$.  We will construct a quasi-conformal map $P \cup A \to Q$ by using two applications of \cite[Theorem 5.1]{buser2014quasiconformal}. 

Let $R$ be a pair of pants where one leg is a cusp, and where $R$ has boundary lengths $0, \ell_1, \ell_2$.  We will define a map $P \cup A \to R$. Recall $P$ is a hyperbolic pair of pants, $A$ is a Euclidean cylinder, and $R$ is a hyperbolic pair of pants.   Then $R$ is noncompact, and strictly contains the union $P' \cup A'$ which is compact.  Here $P' \cap A'$ is a horocycle of length $\frac{2}{\pi} \varepsilon$, and $A'$ is the hyperbolic annulus bounded by horocycles of length $\frac{2}{\pi} \varepsilon$ and corresponding modulus, and $P'$ is the hyperbolic pair of pants with boundary lengths $\frac{2}{\pi} \varepsilon$ and $\ell_1, \ell_2$. 

%Decompose $R= P' \cup A'$ where $P' \cap A'$ is a horocycle of length $\frac{2}{\pi} \varepsilon$.   So $A'$ is a hyperbolic cylinder with boundary horocycles of lengths $\frac{2}{\pi} \varepsilon$ and $\frac{\varepsilon}{L + \frac{\pi}{2}}$ (the cusp).


%\tinytodo{R isn't the union of this $P'$ and $A'$. R is noncompact, the union is compact. you just want to set $A'$ to be the annulus bounded by these horocycles, and then $R$ strictly contains the union.} 
Throughout this proof, the gluing maps are what \cite{buser2014quasiconformal} calls ``boundary coherent," that is they match up on the boundary, and for a homeomorphism $\phi : Y \to Y'$ with boundary curves parametrized by $\alpha_i$ and $\alpha_i'$ respectively, we have $\phi ( \alpha_i (t)) = \alpha'_i (t)$ for $t \in [0,1]$.   Since the maps on pairs of pants are boundary coherent, we will be able to remove a pair of pants and replace it by a different pair of pants with the same boundary lengths using an application of \cite{buser2014quasiconformal}.  This works because the maps on the boundary curves fit together, since the curves are the same length.  All our gluing maps will just be unit speed parametrizations of the boundary horocycles. 

% Also $P'$ is a hyperbolic pair of pants with boundary lengths $\ell_1, \ell_2$ and $\frac{2}{\pi} \varepsilon$.  
An application of \cite[Theorem 5.1]{buser2014quasiconformal} gives a boundary coherent quasi-conformal map $P \to P'$. %\tinytodo{I think one has to be more careful with saying what these maps to along the boundary,  because you are trying to patch the map between the Ps together with a map between the As.} 
We construct a conformal map $A \to A'$ by lifting $A$ to the hyperbolic plane in the upper half space model, so the fundamental domain is a quadrilateral with the horocycle of length $\frac{2}{\pi} \varepsilon$ developed along $y=1$ and a vertical $\frac{2}{\pi}L$ perpendicular to it. %\tinytodo{this sentence is kind of confusing. ``There ..... , so''  makes me think you've already constructed the map. }    
Computing the hyperbolic distance along the top of the fundamental domain, we see that it is $\varepsilon ' = \frac{\varepsilon}{1 + \frac{2}{\pi}L}$.  Thus we may apply \cite[Theorem 5.1]{buser2014quasiconformal} to obtain a quasi-conformal map $Q \to R$ since $Q$ and $R$ have the same boundary lengths: $\ell_1, \ell_2, \varepsilon '$.  The map $Q \to R$ is an embedding, but we can invert it on the compact sub pair of pants in $R$ where we take the boundary horocyle at the cusp to have length $\frac{\varepsilon}{\frac{\pi}{2} +L}$. Composition yields the desired quasi-conformal map $P \cup A \to Q$. 
%\tinytodo{the map $Q \to R$ is just embedding, so you can't invert it. you need to be restricting to some compact sub pair of pants in $R$}

\textbf{Claim}: the map $P \cup A \to Q$ is bi-Lipschitz outside the reduced collar of $c$. 

%\tinytodo{ probably we should just call it the reduced collar and label it RC or something, and maybe call the standard collar $SC(c_+)$. i don't know.} 
Let $\RC(c_+) \subset P$ be the neighborhood of $c_+$ in $P$ with radius $\ln (\frac{2}{\varepsilon})$.  We set $\RC(c_+) = \emptyset$ if $\ell(c_+) \geq 2$.  This is smaller than the standard collar since $\ln (\frac{2}{\varepsilon}) < \sinh ^{-1} (\frac{1}{\sinh(2 \varepsilon)}) $.  In \cite{buser2014quasiconformal} it is called the reduced collar. The authors in \cite{buser2014quasiconformal} show the map $P \to R$ is uniformly bi-Lipschitz except on $\RC(c_+)$.  The image of $P \setminus \RC(c_+)$ is the part of $R$ that lies above the length 1 horocycle around the cusp by \cite{buser2014quasiconformal}{Theorem 5.1 (ii)}.  Similarly, the map $Q \to R$ is uniformly bi-Lipschitz except on the corresponding reduced collar, and the image of $Q \setminus \RC(c_+)$ is the same as above.  Thus $P \setminus \RC(c_+) \to Q$ is uniformly bi-Lipschitz.  In particular, the map from $P \setminus \SC (c_+) \to Q$ is uniformly bi-Lipschitz, since the standard collar $\SC(c_+ ) \supset \RC(c_+)$. 

\textbf{Case 2: $c$ is adjacent to a flare} 

Now suppose $c$ is adjacent to a flare, $F$, and again denote $\varepsilon = \ell(c)$.  Graft a Euclidean cylinder, $A$, to the other side of $c$ of circumference $\varepsilon$ and length $L$.  Note $F \cap A = c$ which has length $\varepsilon$.  Let $Q$ be a hyperbolic flare with base curve of length $\varepsilon ' = \frac{\varepsilon}{1 + \frac{2}{\pi}L}$.  Parametrizing $F = S^1 _ \varepsilon \times [0, \frac{\pi}{2})$, and $A = S^1 _ \varepsilon \times [0, L]$ and $ Q= S^1 _{ \varepsilon'} \times [0, \frac{\pi}{2})$ gives a conformal map $ F \cup A \to Q$, since a quick check shows the moduli are the same: $\frac{\frac{\pi}{2}}{\varepsilon'}= \frac{\frac{\pi}{2} + L}{\varepsilon}  $. Notice these are the same moduli as in the pair of pants case. 

\textbf{Claim:} the map $F \cup A \to Q$ is $4$ bi-Lipschitz on all of $F$. %\tinytodo{might as well include the bilipschitz constant, since it's important that it's uniform, and the constant is like 4 or something}

The conformal map scales by $\frac{1}{1 + \frac{2}{\pi} L}$ in the upper half plane coordinates.  So the Euclidean length distortion is also $\frac{1}{1 + \frac{2}{\pi} L}$.  The hyperbolic metric at a point $(x,y) \in \bbS^1 _ \lambda \times [ 0, \frac{\pi}{2})$ in any hyperbolic cylinder is scaled by $\sec(y)$.  Notice $\frac{1}{2} \cdot \frac{1}{\frac{\pi}{2} -y}. \leq \sec(y) \leq 2 \cdot  \frac{1}{\frac{\pi}{2} -y}$.  Since we are only interested in Lipschitz error we may assume the hyperbolic scaling factor is $\frac{1}{\frac{\pi}{2} -y}$. 

A point in $F = \bbS^1 _ \varepsilon \times [0, \frac{\pi}{2})$ at height $y$ is mapped to a point in $ Q= \bbS^1 _{ \varepsilon'} \times [0, \frac{\pi}{2})$ at height $(L+y) \frac{1}{1 + \frac{2}{\pi}L}$.  So the hyperbolic length distortion of the map $F \cup A \to Q$ restricted to $F$ is within a factor of $2 \cdot 2 =4$ of: the product of the scaling factor of the hyperbolic metric in the image (SHI)  with the Euclidean length distortion (ELD), divided by the scaling factor for the hyperbolic metric in the domain (SHD).  In symbols this is 
\[ \frac{\textrm{(SHI) (ELD) }}{\textrm{(SHD)}} =\frac{   \frac{1}{\frac{\pi}{2} - (L+y) \frac {1}{1+ \frac{2}{\pi} L}} \cdot \frac{1}{1 + \frac{2}{\pi}L} }{\frac{1}{\frac{\pi}{2}-y}}
= \frac{ \frac{\pi}{2}-y }{\frac{\pi}{2}(1 + \frac{2}{\pi} L) -L -y}
=  \frac{ \frac{\pi}{2}-y }{\frac{\pi}{2} +L -L -y} =1.\] 

We have now described the process for each curve $c \in \SSS$.  So we may now create a new surface $Y$ from $X_L$ in the following manner. For each $c \in \SSS$, graft in an annulus, and then replace the appropriate $P \cup A$ or $F \cup A$ with respective quasi-conformal map to the appropriate $Q$.  The replacement maps are boundary coherent by \cite{buser2014quasiconformal} since the boundary lengths remain the same. %\tinytodo{say what the gluing maps are}
%\tinytodo{This sentence doesn't make sense. You  should be cutting out the surfaces $P \cup A$ and $F \cup A$ and replacing them with the associated $Q$ surfaces.  Anyway, probably all of this should be said more rigorously than I do in the file. Like, you need to say what the gluing maps are when you cut out and glue in different pieces.} 
This gives a uniformly quasi-conformal map 
\[f: X_L \to Y \]
where $f$ acts the identity on the complements of the pants and flares $P$ and $F$. %\tinytodo{f isn't the identity, it's the maps you constructed above. it's the identity (suitably interpreted) OUTSIDE these pants and flares.} 
Moreover, on the complements of the standard %\tinytodo{you write regular collar a lot. you mean standard, or reduced?} 
collars of all $c \in \SSS$, the composition 
\[ X \setminus \SSS \xrightarrow{i} X_L \xrightarrow{f} Y \] 
is uniformly locally bi-Lipschitz. 

By Theorem \ref{thm: Hubbard}, there is a map $\delta: \RR_+ \to \RR_+$ which depends only on the quasi-conformal constant (hence just on $M$) so that $f^{-1}$ distorts distances according to $\delta$.  Thus for all $x,y \in X \setminus \SSS$ we have
\[ d_{({X_L})^{\hyp}}(\iota(x), \iota(y)) \geq \delta (d_Y( f \circ \iota (x), f \circ \iota (y))).\] %\tinytodo{you're actually applying Hubbard to $f^{-1}$ here. also, it should be $f \circ i$ everywhere here, not $i \circ f$.}
Now suppose $x,y$ lie outside the standard collars of every $c \in \SSS$ and let $\gamma$ be the shortest path from $f \circ \iota (x) $ to $f \circ \iota (y)$ in $Y$.  Set $Z $ to be $X$ minus the standard collars of $c \in \SSS$.  Then $\gamma$ divides into subpaths which are either contained in $f \circ \iota  (Z)$, or the subpaths have interiors outside $f \circ \iota  (Z)$ .  Denote these as type 1 and type 2 subarcs respectively.  Since $f \circ \iota $ is uniformly bi-Lipschitz on $Z$, then each type 1 subarc is the image of an arc in $X$ whose length only differs by a uniform multiplicative factor.  Notice there are only finitely many such subarcs since the distance between $x$ and $y$ is finite. Every time we traverse a collar we add nonzero length, so the collars can only be traversed finitely many times, and $\gamma$ splits into finitely many subpaths. 

Now, $f \circ \iota  (X)$ is the union of $f \circ \iota (Z)$ with some complementary annuli that are the images of the collars.  Thus type 2 subarcs either have both endpoints in the same boundary component of a complementary annulus $B$, (type 2a), or the endpoints are in two different boundary components of $B$ (type 2b).  Suppose $f \circ \iota  (a) $ and $f \circ \iota (b)$ are endpoints of one such type 2b arc $\alpha$.  Then we claim there is another arc $\beta$ in $X$ connecting $a$ to $b$ and such that
\[ \textrm{length}(\beta) \leq N + N \cdot \textrm{length}(\alpha)  \] 
since the boundary components of $B$ and those of the standard collars of the curves in $\SSS$ have bounded length, and the distance across $B$ is strictly bigger than the distance across the standard collar in $X$. %\tinytodo{this actually needs an argument... } 
This follows from \cite{buser2014quasiconformal} {Theorem 5.1 (ii)} which says that the length of the pinched collar in $Y$ is longer than the length of the standard collar in $X$. \todo{Need help completing argument with the arcs}

Take $N$ to be the minimum of all these lengths of every type of subarc.  Thus iterating over all subarcs, we produce a path in $X$ from $x$ to $y$ with length less than $  N + N \cdot \textrm{length}(\gamma)$. \todo{compute} Therefore 
\[ d_X(x,y) \leq N + N \cdot d _Y(f \circ \iota  (x), f \circ \iota  (y)) \] 
\[ \textrm {thus } \qquad  \delta ^{-1}( \frac{1}{N}( d_X( x,y) -N) ) \leq d_{({X_L})^{\hyp}} ( \iota (x), \iota (y)).   \] 
Thus to finish the proof for surfaces we may take $\eta$ to be the rescaling $\eta(t) = \delta^{-1}  (\frac{1}{N} (t-N) )$. 

\textbf{Now we explain how to modify the proof to cover the case where X is an orbifold.}
One approach would be to modify the proof in \cite{buser2014quasiconformal} to cover generalized pairs of pants, which allow cone points on some of the cuffs.  One can carefully work through all the estimates to do this.  Instead we present a proof using covers. 

The strategy is to pass to a ``good" finite cover $\hat X$ in which we can use the distance comparisons from the surfaces case, and then descend back down to the original orbifold $X$.  Let $\mathcal S \subset X$ a finite collection of curves along which we wish to graft. Let $X_L$ be an orbifold with annuli grafted along all $c \in \mathcal S$.  We will use the finite cover $\hat X$ to compare distances in $X_L$ with those in an orbifold with a uniformized hyperbolic structure. 

We claim there is a finite topological type suborbifold, $Z$, with geodesic boundary, possibly containing flares, and with $\mathcal S \subset \textrm{int} (Z)$.   To find $Z$, extend $\mathcal S$ to a pants decomposition $\mathcal P$ of the interior of the convex core of $X$, using Theorem \ref{thm: pantsdecomps}. 
Then take the hull of all of the pants in $X$ adjacent to curves in $\mathcal S$. 
So we define $Z$ by taking the connected union of finitely many (generalized) pants that includes $\mathcal S$ and append any flares or pants that are adjacent to $\mathcal S$. 
Since $Z$ includes flares and pants with a curve in $\mathcal S$ just along one cuff,  none of the curves in $\mathcal S$ are parallel to boundary components of $Z$.  

Then $Z$ is the union of a compact suborbifold, together with some cusps and flares.   We claim $Z$ contains only finitely many cone points.   There are no cone points on flares or cusps, so if we consider $Z$ with the cusps and flares amputated, then it is a compact suborbifold (possibly with boundary).  A compact suborbifold contains only finitely many cone points.   Cone points cannot accumulate, and every embedded annulus in $Z$ contains only finitely many cone points.  Thus $Z$ contains finitely many cone points. 
%
By Proposition \ref{prop: finitecovers}, $Z$ has a finite cover $\hat Z$ where every cone point has a smooth lift. 




Let $\hat {\mathcal S} \subset \hat Z \subset \hat X$ be the lift of $\mathcal S$.  Then we can extend $\hat {\mathcal S}$ to a pants decomposition of $\hat X$.  Then $\hat Z$ is a finite type subsurface, and contains $\hat {\mathcal S}$.    Recall $L: X \to X_L$ grafts in annuli of length $L_i$ along each curve $c_i \in \mathcal S$.  We take the pullback $\hat L: \hat X \to \hat X_L$ which grafts in an annulus of length $L_i$ along every lift $\hat c_i \in \hat { \mathcal S}$ of $c_i \in \mathcal S$.  Thus the map $\hat L: \hat X \to \hat X_L$ covers the map $L : X \to X_L$.  If $c_i \in \mathcal S$ is nondegenerate, then the annuli grafted at $ \hat c_i$ map isometrically to the annuli grafted at $c_i$.  If $c_i \in \mathcal S$ is degenerate, then the annuli grafted at $\hat c_i$ double cover the annuli grafted at $c_i$. 


Now $\hat Z$ is a finite type surface and contains every curve in $\hat {\mathcal S}$.  Let $\hat Z_L$ be the finite type surface which contains all annuli grafted along curves in $\hat {\mathcal S}$.  Since $\hat Z$ is a finite type subsurface we may apply \cite{buser2014quasiconformal} as in the argument in the proof for surfaces to find a quasiconformal map $\hat f$ from $\hat Z_L$ to some $\hat W $ which is a hyperbolic finite type surface.  Notice $\hat f$ affects only pairs of pants or flares adjacent to curves in $\hat {\mathcal S}$, and $\hat f$ is the identity on pants and flares that are not adjacent to curves in $\hat {\mathcal S}$.  Thus we may extend $\hat f : \hat X_L \to \hat Y$ where $\hat Y$ is an orbifold with hyperbolic structure where we have removed $\hat Z_L$ and replaced it with $\hat W$.  



To finish the proof we need to compare distances in $X$ and $Y$. Take $x,y \in X$, and let $\alpha$ be a path from $x$ to $y$ in $X$. Lift $\alpha$ to a curve $\hat{\alpha}$ to $\hat{X}$, and let $\hat{x},\hat{y}$ be its endpoints. By the first part of the proof for surfaces, we know applied to $\hat X_L$ we know $ d_{({\hat{X}_L})^{\hyp}}(\iota(\hat x), \iota(\hat y)) \geq \hat \eta (d_{\hat{X}}(\hat x,\hat y))$ for some function $\hat \eta$.   Thus there is a path $ \hat \beta$ from $\hat x $ to $\hat y$ in $\hat Z \subset \hat X$ and $\hat \beta$ minimizes the distance between $\hat x, \hat y$ in $\hat X$. Thus $\ell (\hat \beta) \leq \ell ( \hat \alpha)$.   Then $\beta$ projects to a path in $Z \subset X$ which minimizes the distance between $x$ and $y$, so $\ell( \beta) \leq \ell ( \alpha)$.  The conclusion follows. 
\end{proof}


==> weils_graveyard.tex <==
I am weeping. It is so painful to see this go aWeil, but there is no reason to include it anymore.



\subsection{Representation Varieties, Teichm\"uller space and Moduli space}
Let $\mathcal R(S)$ be the \emph{representation variety} consisting of all type preserving representations $\pi_1 S \longrightarrow G$, where type preserving means that peripheral elements of $\pi_1 S$ map to parabolic elements of $G $. If we choose a finite presentation for $\pi_1 S$, say of the form 
\[\pi_1 S = \langle \  a_1,b_1,\ldots,a_g,b_g,c_1,\ldots,c_k,d_1,\ldots,d_l \ \ | \ \  c_i^{n_i}, \ \prod_i [a_i,b_i] \prod_i c_i \prod_i d_i \  \rangle,
\]
where here the $c_i$ correspond to cone points, and the $d_i$ to punctures, then $\mathcal R  (S) $ can be considered as a subvariety of $G^{2g+k+l}$ cut out by equations corresponding to the relations above and the condition that all the $d_i$ map to parabolics. 

Let $\mathcal {DF}(S) \subset \mathcal R(S)$ be the set of all discrete, faithful representations. By for instance a result of Bergeron-Gelander \cite[Theorem 1.1]{bergeron2004note}, the set $\mathcal {DF}(S)$ is an open subset of $\mathcal R(S)$, where we consider the later with the induced topology from $G^{2g+k+l}$, i.e.\ the topology of pointwise convergence of representations. See Kapovich \cite{kapovich2001hyperbolic} for more information on representation varieties. 

\begin{lemma}[\S 4--7 in Weil \cite{weil1964remarks}]
$\mathcal {DF}(S)$ is a smooth submanifold of $G^{2g+k+l}$ of dimension $6g+2k+2l-3$.
\end{lemma}

The main ideas are in the paper cited above, but we sketch the argument the result is not stated as such there, and we could not find another reference that applies in this generality. Note that the dimension of $\mathcal {DF}(S)$ is what you would expect from counting the number of equations above that cut out $\mathcal R(S) \subset G^{2g+k+l}$. Namely, the condition $c_i^{n_i}=1$ is equivalent to requiring that $c_i$ map to the codimension $1$ set of order $n_i$ elliptics in $G$, the type preserving condition requires that each $d_i$ map to the codimension $1$ set of parabolics, and the final relator imposes a codimension $3$ condition. So, the dimension of $\mathcal R(S)$ should be $$3(2g+k+l) - k - l - 3 = 6g+2k+2l-3.$$

\begin{proof}[Proof Sketch] 
We start by following \S 7 in \cite{weil1964remarks}, altering it to allow for cusps. The torsion relations and the type preserving conditions imply that $\mathcal R(S)$ is contained in the subset \[G^{2g} \times E_1 \times \cdots \times E_k \times P^l \subset G^{2g+k+l},\]
where $E_i \subset G$ is the $2$-submanifold consisting of order $n_i$ elements and $P\subset G$ is the $2$-submanifold of parabolic elements. The final relator in our presentation then can be considered as a smooth map
\[ \Phi : G^{2g} \times E_1 \times \cdots \times E_k \times P^l \longrightarrow G,
\] where $\mathcal R(S) = \Phi^{-1}(1)$. At a given representation $\rho \in \mathcal R(S)$, the kernel $\ker d\Phi_\rho$ is the space of \emph {parabolic co-cycles} associated to $\rho $ that Weil discusses in \S 5. Briefly, a $1$-cocycle is a map $z : \pi_1 S \longrightarrow \mathfrak g$ such that $z(\gamma \gamma') = z(\gamma) + Ad(\rho(\gamma))z(\gamma')$ for all $\gamma,\gamma'\in \pi_1 S$, and $z$ is \emph{parabolic} if all $z(c_i) $ and $z(d_i)$ lie in the images of the linear maps $1-Ad(\rho(c_i))$ and $1-Ad(\rho(d_i))$, respectively. Here, the cocycle condition says that $z$ is obtained by differentiating a path of \emph {representations} starting at $\rho$, rather than an arbitrary path in $G^{2g+k+l}$, and the parabolic condition ensures that the values of $\rho(c_i)$ and $\rho(d_i)$ are just conjugated along the path, which is exactly what you need to say that the path lies in $G^{2g} \times E_1 \times \cdots \times E_k \times P^l$. 
Now equation (19) on pg 155 of \cite{weil1964remarks} says that the  space of parabolic co-cycles has dimension 
\[P=(2g-1)\cdot 3 + i' + \sum_{i=1}^k \mathrm{Rank(1-Ad(\rho(c_i)
)} + \sum_{i=1}^l \mathrm{Rank(1-Ad(\rho(d_i))}.
\] 
Here, our notation is slightly different from Weil's, but we would like to stress that the equation above does actually allow for parabolics: they correspond to the $s_v=0$ case in that section. As stated at the bottom of Weil's pg 155, the factor $i'$ is the dimension of the space of vectors in the dual $\mathfrak g^*$ that are invariant under $\rho(\gamma)^*$ for all $\gamma \in \pi_1 S$. When $\rho$ is nonelementary, so in particular when $\rho \in \mathcal {DF}(S)$, we have $i'=0$. Finally, one can compute directly that the ranks above equal $2$, just by analyzing separately the adjoint actions of elliptic and parabolic elements on the Lie algebra $\mathfrak g$. So, we get that 
\[\dim \ker d\Phi_\rho = 6g + 2k + 2l -3, \ \ \forall \rho\in \mathcal {DF}(S).\]
As this is exactly the dimension of the domain of $\Phi$ minus the dimension of the co-domain, it follows that $\Phi$ has full rank at each point of the open subset $\mathcal {DF}(S) \subset \mathcal R(S) = \Phi^{-1}(1)$. Hence, $\mathcal {DF}(S)$ is a smooth submanifold of $G^{2g+k+l}$ of the stated dimension.
\end{proof}

Regard $G$ as the group of orientation preserving isometries of $\HH^2$. Then $G < \mathrm{Isom}(\HH^2)$ is an index 2 normal subgroup, so $\mathrm{Isom}(\HH^2)$ acts on $G$ by conjugation, and hence acts from the left on $\mathcal {DF}(S)$ via \[\rho(\cdot) \overset{g}{\longmapsto} g \rho(\cdot) g^{-1}, \ \rho \in \mathcal {DF}(S), g \in \mathrm{Isom}(\HH^2). \] The orbit space $\mathrm{Isom}(\HH^2) \backslash \mathcal {DF}(S) $ can be identified with the \emph{Teichm\"uller space} 
\[ \mathcal{T}(S) \cong \big \{\ (X,h) \ \ \big |\  \ h : S \longrightarrow X \text{ a homeo, } X \text { finite volume hyperbolic } \big \} \modsim, \]
where here $(X,h)\sim (X',h')$ if there is an isometry $f : X \longrightarrow X'$ with $(h')^{-1} \circ f \circ h$ homotopic to the identity map. Indeed, any representation $\rho : \pi_1 S \longrightarrow G$ in $\mathcal{DF}(S)$ gives a finite volume quotient orbifold $$X := \rho(\pi_1 S) \backslash \HH^2$$ together with an isomorphism $\pi_1 S \overset{\rho}{\longrightarrow} \rho(\pi_1 S) \cong \pi_1 X$, which determines a homotopy class of markings, and the resulting pair $(X,h)$ only depends on $\rho$ up to the action of $\mathrm{Isom}(\HH^2)$. For details, we refer the reader to the proof of Proposition 10.2 in \cite{primer}; although there $S$ is a closed surface, the proof is exactly the same for finite volume orbifolds. Also, above it is most natural to consider the set $\mathrm{Isom}(\HH^2) \backslash \mathcal {DF}(S)$ with the quotient topology; it is well known that this agrees under the identification with $\mathcal T(S)$ with all the usual definitions of the topology on Teichm\"uller space, e.g.\ by quasiconformal maps. \todo{should figure out what to say here.} The \emph {moduli space} $\mathcal M(S)$ is the set of all isometry classes of finite volume hyperbolic $2$-orbifolds homeomorphic to $S$. It is the quotient of $\mathcal T(S)$ by the mapping class group $\mathrm{Mod}(S)$, and alternatively can be viewed as the space of double cosets \[ \mathrm{Isom}(\HH^2) \backslash \mathcal {DF}(S) / \mathrm{Aut}(\pi_1 S).\] \todo{and here... about the topology.}




